Exact and Metaheuristic Approaches for the Production Leveling Problem

In this paper we introduce a new problem in the field of production planning which we call the Production Leveling Problem. The task is to assign orders to production periods such that the load in each period and on each production resource is balanced, capacity limits are not exceeded and the orders' priorities are taken into account. Production Leveling is an important intermediate step between long-term planning and the final scheduling of orders within a production period, as it is responsible for selecting good subsets of orders to be scheduled within each period. A formal model of the problem is proposed and NP-hardness is shown by reduction from Bin Backing. As an exact method for solving moderately sized instances we introduce a MIP formulation. For solving large problem instances, metaheuristic local search is investigated. A greedy heuristic and two neighborhood structures for local search are proposed, in order to apply them using Variable Neighborhood Descent and Simulated Annealing. Regarding exact techniques, the main question of research is, up to which size instances are solvable within a fixed amount of time. For the metaheuristic approaches the aim is to show that they produce near-optimal solutions for smaller instances, but also scale well to very large instances. A set of realistic problem instances from an industrial partner is contributed to the literature, as well as random instance generators. The experimental evaluation conveys that the proposed MIP model works well for instances with up to 250 orders. Out of the investigated metaheuristic approaches, Simulated Annealing achieves the best results. It is shown to produce solutions with less than 3% average optimality gap on small instances and to scale well up to thousands of orders and dozens of periods and products. The presented metaheuristic methods are already being used in the industry.

==> Production Leveling Technical Report/definitions.tex <==
\usepackage{todonotes}
\usepackage{amsthm, amsmath}
\usepackage{tabularx, booktabs, paralist}
\usepackage{diagbox}
\usepackage{multirow}
\usepackage{subcaption}

% \usepackage[cache=false]{minted}
\usepackage[ruled,linesnumbered]{algorithm2e} % can use algochapter if chapters are defined
\LinesNumbered

\usepackage{nicefrac}

\usepackage[acronym,toc]{glossaries}
% \makeglossaries

%Macros
%environemnts for theorems etc.
\newtheorem{theorem}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{example}{Example}

%Environemnt for computational problems
%decision problems
\newcommand{\cprob}[3]{
\begin{center}
{\small
\begin{tabularx}{0.98\columnwidth}{ll}
\toprule
\multicolumn{2}{c}{\textsc{#1 (Decision problem)}} \\
\midrule
\textbf{Instance}:   & \parbox[t]{0.8\columnwidth}{#2\vspace*{1mm}}  \\
\textbf{Question}:   & \parbox[t]{0.8\columnwidth}{#3\vspace*{.5mm}} \\
\bottomrule
\end{tabularx}
}
\end{center}
} 
%optimization problems without constraints
\newcommand{\optprob}[3]{
\begin{center}
{\small
\begin{tabularx}{0.98\columnwidth}{ll}
\toprule
\multicolumn{2}{c}{\textsc{#1 (Optimization problem)}} \\
\midrule
\textbf{Instance}:   & \parbox[t]{0.8\columnwidth}{#2\vspace*{1mm}}  \\
\textbf{Question}:   & \parbox[t]{0.8\columnwidth}{#3\vspace*{.5mm}} \\
\bottomrule
\end{tabularx}
}
\end{center}
} 
%optimization problems with constraints
\newcommand{\optprobc}[4]{
\begin{center}
{\small
\begin{tabularx}{0.98\columnwidth}{ll}
\toprule
\multicolumn{2}{c}{\textsc{#1 (Optimization problem)}} \\
\midrule
{\bf Instance:}   & \parbox[t]{0.8\columnwidth}{#2\vspace*{1mm}}  \\
{\bf Objective:}& \parbox[t]{0.8\columnwidth}{#3\vspace*{.5mm}} \\
{\bf Constraints:}& \parbox[t]{0.8\columnwidth}{#4\vspace*{.5mm}} \\
\bottomrule
\end{tabularx}
}
\end{center}
} 

% Complexity classes
\newcommand{\NP}{$\mathcal{NP}$}
\newcommand{\Ptime}{$\mathcal{P}$}

% Acronyms
\newacronym{plp}{PLP}{Production Leveling Problem}
\newacronym{bacp}{BACP}{Balanced Academic Curriculum Problem}
\newacronym{salb}{SALB}{Simple Assembly Line Balancing}
\newacronym{tps}{TPS}{Toyota Production System}
\newacronym{mip}{MIP}{Mixed Integer Programming}
\newacronym{cp}{CP}{Constraint Programming}
\newacronym{sos1}{SOS1}{Specially Ordered Set Type 1}
\newacronym{vnd}{VND}{Variable Neighborhood Descent}
\newacronym{vns}{VNS}{Variable Neighborhood Search}
\newacronym{smac}{SMAC}{Sequential Model-based Algorithm Configuration}



==> Production Leveling Technical Report/methods/mip-model.tex <==
\begin{align}
\textsf{min}\hspace{1cm} & a_1 g_1 + a_2 g_2 + a_3 g_3 && \label{ex8:1}\\
\textsf{s.t.}\hspace{1cm} & \sum_{i \in N} x_{ij} = 1							& j \in K 				  \label{eq:mip_one_x}\\
						  & \sum_{i \in N} i \cdot x_{ij} = y_j 				& j \in K 			      \label{eq:mip_link_xy}\\
						  & y_i - y_j \leq (n-1) z_{ij}							& i, j \in K \enspace\vert\enspace p_i > p_j \label{eq:mip_link_yz}\\
						  & \sum_{j \in K} d_j x_{ij} + s_i^+ - s_i^- = d^*   	& i \in N         \label{eq:mip_slack_constr}\\
						  & \sum_{j \in K | t_j = t} d_j x_{ij}  + s_{it}^+ - s_{it}^- = d_t^*    & i \in N, \enspace t \in M \label{eq:mip_slack_p_constr}\\
						  & d^* + s_i^+ \leq c      							& i \in N 			         \label{eq:mip_cmax_total}\\
						  & d_t^* + s_{it}^+ \leq c_t   						& i \in N, \enspace t \in M \label{eq:mip_cmax[p]}\\
						  & y_i \leq y_j                                        & i, j \in S, S \subseteq {K} \enspace\vert\enspace p_i \geq p_j, d_i = d_j, t_i = t_j \label{eq:mip_symmetry} \\
						  & \sum_{t \in M} (s_{it}^- - s_{it}^+) = s_i^- - s_i^+   & i \in N \label{eq:mip_link_slacks}
\end{align}

